A Tattered Cloak of Invisibility: Measuring Anonymity Loss in Railgun on Ethereum

From a user's perspective, perhaps the most significant difference between traditional banking services and widely used blockchain-based financial systems is that, in the latter, transactions and, either directly or indirectly, account balances and transaction histories are publicly observable. Therefore, a growing number of cryptographic solutions have been proposed to add a privacy layer to such systems. However, the privacy that users actually obtain does not depend solely on the security of the underlying cryptographic protocol: user behavior, transaction amount patterns, and timing decisions can substantially reduce anonymity. In this work, we study behavioral leakage in cryptocurrency mixers, focusing on Railgun on Ethereum. We aim to heuristically estimate the probability that a given deposit and withdrawal transaction belong to the same user. We consider five sources of leakage: characteristic timing patterns, address reuse, proximity in the transaction graph induced by prior public transactions, amount fingerprints that preserve distinctive digit patterns across transaction values, and knapsack type matches in which groups of transaction amounts add up in revealing ways. Our results show that even cryptographically strong privacy systems may suffer substantial anonymity loss due to user behavior and transaction patterns. Our five heuristics are able to uniquely link 17.65% of Railgun withdraw transactions to deposit transactions. We also applied a knapsack solver algorithm that was able to produce a 3.42 bit median anonymity loss for withdraw transactions. This work contributes to a better understanding of the practical privacy limits of mixers and anonymity pools, and points toward safer usage practices and design principles.

==> Figures/figure_ch5_wC_window_scan_1tok_step0.0001_tikz.tex <==
% TIKZ-AFT26: Figure W-C (1tok, step = 0.0001 ETH): ΔH vs matching window
% Data: figure_ch5_wC_window_scan_1tok_step0.0001.csv
% Host documents can override these before \input/\includestandalone.
\makeatletter
\@ifundefined{figurewidth}{\newlength{\figurewidth}}{}
\ifdim\figurewidth=0pt
  \ifdim\linewidth=0pt
    \setlength{\figurewidth}{14cm}
  \else
    \setlength{\figurewidth}{\linewidth}
  \fi
\fi
\@ifundefined{figureheight}{\newlength{\figureheight}}{}
\ifdim\figureheight=0pt
  \ifdim\linewidth=0pt
    \setlength{\figureheight}{7.7cm}
  \else
    \setlength{\figureheight}{0.55\linewidth}
  \fi
\fi
\@ifundefined{TikzAFTDataPath}{\@ifundefined{currfiledir}{\def\TikzAFTDataPath{Figures/}}{\edef\TikzAFTDataPath{\currfiledir}}}{}
\makeatother
\definecolor{cwithdraw}{RGB}{213,94,0}
\definecolor{corange}{RGB}{230,159,0}
\definecolor{csky}{RGB}{86,180,233}
\definecolor{cdeposit}{RGB}{0,158,115}
\definecolor{cteal}{RGB}{68,170,153}
\definecolor{cblue}{RGB}{0,114,178}
\definecolor{cgray}{RGB}{127,127,127}

\begin{tikzpicture}
  \begin{axis}[
    width=\figurewidth, height=\figureheight,
    symbolic x coords={3 d, 7 d, 30 d, all-time},
    xtick=data,
    xlabel={Matching window},
    ylabel={Per-target $\Delta H = \log_2(\#\,\text{pool addr}) - H_{\mathrm{knap,addr}}$ [bits]},
    ymin=0,
    ymajorgrids,
    legend style={at={(0.02,0.98)}, anchor=north west, font=\scriptsize},
  ]
    \addplot[csky, mark=triangle*, mark size=1.8pt, dashed, line width=0.9pt]
      table [col sep=comma, x=window, y=p10_dH] {\TikzAFTDataPath figure_ch5_wC_window_scan_1tok_step0.0001.csv};
    \addlegendentry{p10 $\Delta H$}
    \addplot[csky, mark=triangle*, mark size=1.8pt, dashed, line width=0.9pt]
      table [col sep=comma, x=window, y=p90_dH] {\TikzAFTDataPath figure_ch5_wC_window_scan_1tok_step0.0001.csv};
    \addlegendentry{p90 $\Delta H$}
    \addplot[cblue, mark=*, mark size=2.8pt, line width=1.6pt]
      table [col sep=comma, x=window, y=median_dH] {\TikzAFTDataPath figure_ch5_wC_window_scan_1tok_step0.0001.csv};
    \addlegendentry{median $\Delta H$}
    \addplot[corange, mark=square*, mark size=2.3pt, dotted, line width=1.1pt]
      table [col sep=comma, x=window, y=mean_dH] {\TikzAFTDataPath figure_ch5_wC_window_scan_1tok_step0.0001.csv};
    \addlegendentry{mean $\Delta H$}
  \end{axis}
\end{tikzpicture}

==> Figures/figure_ch5_wC_window_scan_kto1_step0.0001_tikz.tex <==
% TIKZ-AFT26: Figure W-C (kto1, step = 0.0001 ETH): ΔH vs matching window
% Data: figure_ch5_wC_window_scan_kto1_step0.0001.csv
% Host documents can override these before \input/\includestandalone.
\makeatletter
\@ifundefined{figurewidth}{\newlength{\figurewidth}}{}
\ifdim\figurewidth=0pt
  \ifdim\linewidth=0pt
    \setlength{\figurewidth}{14cm}
  \else
    \setlength{\figurewidth}{\linewidth}
  \fi
\fi
\@ifundefined{figureheight}{\newlength{\figureheight}}{}
\ifdim\figureheight=0pt
  \ifdim\linewidth=0pt
    \setlength{\figureheight}{7.7cm}
  \else
    \setlength{\figureheight}{0.55\linewidth}
  \fi
\fi
\@ifundefined{TikzAFTDataPath}{\@ifundefined{currfiledir}{\def\TikzAFTDataPath{Figures/}}{\edef\TikzAFTDataPath{\currfiledir}}}{}
\makeatother
\definecolor{cwithdraw}{RGB}{213,94,0}
\definecolor{corange}{RGB}{230,159,0}
\definecolor{csky}{RGB}{86,180,233}
\definecolor{cdeposit}{RGB}{0,158,115}
\definecolor{cteal}{RGB}{68,170,153}
\definecolor{cblue}{RGB}{0,114,178}
\definecolor{cgray}{RGB}{127,127,127}

\begin{tikzpicture}
  \begin{axis}[
    width=\figurewidth, height=\figureheight,
    symbolic x coords={3 d, 7 d, 30 d, 180 d, all-time},
    xtick=data,
    xlabel={Matching window},
    ylabel={Per-target $\Delta H = \log_2(\#\,\text{pool addr}) - H_{\mathrm{knap,addr}}$ [bits]},
    ymin=0,
    ymajorgrids,
    legend style={at={(0.02,0.98)}, anchor=north west, font=\scriptsize},
  ]
    \addplot[csky, mark=triangle*, mark size=1.8pt, dashed, line width=0.9pt]
      table [col sep=comma, x=window, y=p10_dH] {\TikzAFTDataPath figure_ch5_wC_window_scan_kto1_step0.0001.csv};
    \addlegendentry{p10 $\Delta H$}
    \addplot[csky, mark=triangle*, mark size=1.8pt, dashed, line width=0.9pt]
      table [col sep=comma, x=window, y=p90_dH] {\TikzAFTDataPath figure_ch5_wC_window_scan_kto1_step0.0001.csv};
    \addlegendentry{p90 $\Delta H$}
    \addplot[cblue, mark=*, mark size=2.8pt, line width=1.6pt]
      table [col sep=comma, x=window, y=median_dH] {\TikzAFTDataPath figure_ch5_wC_window_scan_kto1_step0.0001.csv};
    \addlegendentry{median $\Delta H$}
    \addplot[corange, mark=square*, mark size=2.3pt, dotted, line width=1.1pt]
      table [col sep=comma, x=window, y=mean_dH] {\TikzAFTDataPath figure_ch5_wC_window_scan_kto1_step0.0001.csv};
    \addlegendentry{mean $\Delta H$}
  \end{axis}
\end{tikzpicture}

==> old.tex <==
\section{Deanonymization Heuristics}\label{sec:heuristics}
While Railgun cryptographically obscures the details of chain transactions, adversaries can employ statistical and behavioral heuristics to deanonymize a user. These heuristics may exploit patterns, system-level weakness on zero-knowledge-based systems, and may possibly use metadata leaks. Common attack vectors may include time-of-transaction correlation, gas fingerprinting, address reuse across protocols, and graph-theoretic clustering of interacting accounts. This section aims to analyze some of those heuristics that threaten Railgun's privacy guarantees evaluating their theoretical and practical prevalence in Ethereum's ecosystem. Each heuristics is examined through real world cases followed by Railgun's countermeasures.
\subsection{Transaction between Deposit and Withdraw addresses}
To qualify address reuse within Railgun's privacy preserving system, the initial approach involved collecting deposit and withdrawal data through Etherscan's API. However, tow main limitations hindered this method: The Api's inability to differentiate shielded from regular transactions, and a strict pagination limit (10,000 results), which resulted in incomplete coverage of the data.
To overcome these obstacles, the analysis was adapted to Dune Analytics, which offers access to community-curated blockchain datasets. Specifically, the study utilized \texttt{erc20\_ethereum.evt\_Transfer} for general ERC-20 token transactions and \texttt{dune.coldfire\_team.result\_railgun\_withdrawals\_v\_2} which tracks Railgun specific withdrawals. A total of 25,000 transactions between 2022 and 2025 were extracted and analyzed.
A key objective was to measure the extent of address reuse between deposits and withdrawals. The analysis revealed approximately 7-10\% of transactions involved the same addresses being used for deposit and withdrawal transactions suggesting that a non-negligible portion of users do not fully utilize the privacy guarantees offered by Railgun.
In support of these findings, Figure~\ref{fig:fractional_parts} shows the distribution of fractional parts of deposit and withdrawal amounts. These distributions reveal distinct spikes at around numbers (e.g. 0.0, 0.5, and.99), particularly in withdrawals.This suggests that some users are manually specifying amounts that follow recognizable patterns. These patterns may reduce the entropy of the system, potentially helping to deobfuscate or link analysis.
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{Figure_1.png}
    \caption{Distribution of fractional parts in deposit (left) and withdrawal (right) amounts. Noticeable spikes at 0.0, 0.5, and 0.99 suggest behavioral patterns or automation.}
    \label{fig:fractional_parts}
\end{figure}
\subsection{Gas fee fingerprints}g
To further investigate potential linkage between Railgun deposit and withdrawal transactions, this study introduces the Gas Fee Fingerprint heuristic, which uses high prevision decimal values as identifiers.
The underlying intuition is based on the observation that values beyond a certain decimal precision (e.g., 0.00000001) have negligible economic impact and are often preserved across multiple related transactions. For instance, a deposit of 2.00000123 and a withdrawal of 1.450000123 may be heruistically linked via the.00000123 fingerprint, suggesting they may originate from the same user or wallet.
This pattern arises because micro values are unlikely to be chosen arbitrarily by unrelated users. Insted they often emerge from:
\begin{enumerate}
  \item \textbf{Wallet rounding behavior}
  \item \textbf{Custom withdrawal scripts}
  \item \textbf{Dust values left after fees}
\end{enumerate}

By extracting and comparing the fractional components of both deposit and withdrawal values, 91,385 transactions were analyzed using this method. This proved useful in narrowing down candidate withdrawal addresses for specific deposits. Ultimately, reducing the anonymity set for those transactions. Although this may seem insignificant, this approach serves as a probabilistic linking mechanism that can be further strengthened when combined with other heuristics (e.g., address reuse).
This technique highlights an impactful risk in privacy system where even insignificant values can leak identity or linkage information across shielded and unshielded domains

\subsection{Subset sum analysis}
The Subset sum Analysis is a deanonymization heuristic that exploits the additive nature of financial transactions. The core idea being to identify combinations of withdrawal amounts that when summed closely match prior amounts. This heuristic assumes that a single deposit might later be split across multiple withdrawals. A behavior that is very commonly observed in real world usage of privacy systems like Railgun or Tornado Cash.

This technique is effective in scenarios where:

\begin{enumerate}
  \item \textbf{Users split a large deposit into smaller, structured withdrawals.}
  \item \textbf{The withdrawal amounts exhibit low entropy (e.g., round numbers or known values).}
  \item \textbf{The time window between the deposit and related withdrawals is short, limiting the search space.}
\end{enumerate}

For example, let's say a user deposits \textbf{5.7321 ETH} into Railgun. Later we found three withdrawals of \textbf{2.0 ETH}, \textbf{1.7321 ETH} and \textbf{2.0 ETH}. The exact sum \textbf{5.7321 ETH} suggests that these withdrawals may have originated from the same deposit, even if done over multiple addresses. This weakens anonymity by linking seemingly unrelated withdrawals.

To perform subset sum analysis at scale the following technique was used:
\begin{enumerate}
  \item \textbf{Enumerate deposit amounts within a selected time window.}
  \item \textbf{Extract sets of withdrawals that occur after each deposit.}
  \item \textbf{Use an optimized subset sum algorithm to find combinations of withdrawals that approximate the deposit amount.}
  \item \textbf{Flag any matches as potential linkage candidates.}
\end{enumerate}

This heuristic becomes more potent when combined with the following:
\begin{enumerate}
  \item \textbf{Timestamp proximity:} Filtering withdrawals that occur soon after a deposit.
  \item \textbf{Amount fingerprinting:} Prioritizing combinations involving unique fractional parts.
  \item \textbf{Relayer reuse:} Identifying common relayers across transactions.
\end{enumerate}

Although subset sum does not directly deanonymize a user, it is a powerful probabilistic technique that reduces the anonymity set by filtering feasible linkage candidates. It's effectiveness scales with the number of structured or repeated withdrawal behavior among users.



\section{Heuristics Evaluation and Measurements}\label{sec:evaluation}

In this section, we  evaluate the effectiveness of the deanonymization heuristics outlined above using real-world Railgun data extracted from Ethereum mainnet. Each heuristic was tested with on-chain events and analyzed for both theoretical impact and practical prevalence.

\subsection{Address Usage in Deposit and Withdrawal}\label{sec:heuristic1}

The first and simplest heuristic targets \textbf{address reuse} across deposit (shield) and withdrawal (unshield) transactions. In Railgun, privacy is maximized when users employ fresh addresses for every interaction. However, convenience, poor wallet design, or user inattention can result in the same address being used for both depositing and withdrawing.

To quantify this risk, we compared all observed deposit and withdrawal addresses in the Railgun pool. Our analysis found that approximately 7.5\% of deposit addresses were also reused for withdrawal (see Figure~\ref{fig:address_reuse_pie}). This non-trivial overlap demonstrates that a measurable portion of the user base undermines their privacy, making their Railgun transactions vulnerable to straightforward linkage attacks.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\textwidth]{1.png}    \caption{Deposit addresses in Railgun: the fraction reused for withdrawal (orange) vs.\ those only used for deposit (gray).}
    \label{fig:address_reuse_pie}
\end{figure}

Such address reuse exposes users to deanonymization, especially if their reused address is linked to external activity (e.g., exchange KYC or other DeFi protocols). This highlights the need for better user education and wallet UI design to enforce best privacy practices.

\subsection{Transactions Between Deposit and Withdrawal Address}\label{sec:heuristic2}

The second heuristic investigates \textbf{direct transactions between deposit and withdrawal addresses}. Even when addresses are not reused, on-chain activity outside of Railgun can reveal relationships between them. For example, if a deposit address later sends ETH or tokens directly to a withdrawal address, or vice versa, an adversary can infer that the same entity may control both.

To evaluate this heuristic, we scanned all Ethereum transactions between addresses observed as Railgun depositors and withdrawers. We found that a small but non-negligible subset of address pairs were linked by direct transfers, either before or after their use in Railgun. Figure~\ref{fig:direct_txn_bar} visualizes the counts of such direct transactions (deposit $\rightarrow$ withdraw and withdraw $\rightarrow$ deposit) among observed address pairs.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\textwidth]{2.png}    \caption{Number of on-chain direct transactions between deposit and withdrawal addresses used in Railgun.}
    \label{fig:direct_txn_bar}
\end{figure}

The presence of such links provides a powerful deanonymization tool for adversaries, as it connects otherwise shielded Railgun transactions to public activity on Ethereum. For maximal privacy, users should avoid any on-chain connections between addresses used with Railgun.

\subsection{Transaction Fee Fingerprinting}\label{sec:heuristic3}

The third heuristic leverages \textbf{transaction fee fingerprinting}, focusing on the fine-grained decimal “fingerprints” left by gas or relayer fees. Since fees are often specified to high decimal precision (sometimes due to wallet rounding, relayer behavior, or custom scripts), rare or unique fee patterns can be used to link deposits and withdrawals.

We analyzed all withdrawal transactions in WETH, extracting the fractional part of the relayer fee to 8 decimal digits. Most fee fingerprints were unique or extremely rare, as shown in Figure~\ref{fig:relayer_fee_histogram}. This suggests that even micro-value leakages can serve as probabilistic linkage points between shielded and unshielded activity.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\textwidth]{3.png}    \caption{Distribution of relayer fee decimal fingerprints (8 decimal digits) for WETH withdrawals. Most fingerprints are unique or rare, increasing linkage risk.}
    \label{fig:relayer_fee_histogram}
\end{figure}

By cross-referencing rare fee fingerprints across deposits and withdrawals, adversaries can narrow down possible matches and, in some cases, deanonymize users. This result underscores the importance of protocol-level countermeasures such as enforced fee rounding or user interface guidance to avoid accidental fingerprinting.

\subsection{Summary}
Our evaluation shows that all three heuristics—address reuse, direct transaction linkage, and transaction fee fingerprinting—are observable in practice and have measurable impact on Railgun’s privacy guarantees. The strongest attacks combine these signals, significantly shrinking the anonymity set for affected users.

\section{Countermeasures}\label{sec:countermeasures}
While Railgun uses zero-knowledge profs to preserve transaction privacy, our analysis highlights that behavioral and statistical heuristics can still reveal a lot of common linkage between deposits and withdrawals. To increase anonymity guarantees, this section outlines countermeasures of practical and theoretical concepts for each identified heuristic.

\subsection{Address Reuse Mitigation}
One of the most direct privacy leaks arises from users reusing the same wallet address for both deposit and withdrawal transactions. This practice undermines the core value of anonymity by linking shielded and public identities.
\textbf{Recommended Countermeasures:}
\begin{itemize}
    \item \textbf{Default Enforcement of One-Time Addresses:} Clients should discourage or prevent reuse of addresses, particularly for withdrawals. Integration of automatic address rotation mechanisms in wallet interfaces could make this behavior the default
    \item \textbf{Wallet Warning and UX Nudges:} User interfaces should display clear warnings when a previously used address is selected for a withdrawal.
\end{itemize}

\subsection{Mitigating Gas Fee Fingerprints}
High-precision decimal patterns can act as pseudo-identifiers across transactions. These arise from microvalue residues due to rounding or fee calculations, unintentionally linking deposits to corresponding withdrawals.
\textbf{Recommended Countermeasures:}
\begin{itemize}
    \item \textbf{Standardized Amount Masking:} Introduce configurable rounding or truncating layers in the wallet frontend to eliminate overly precise amounts in deposits and withdrawals.
    \item \textbf{Fee Obfuscation:} Add a small amount of random padding to transaction amounts or fees to reduce recognizability, without compromising user intent or value transfer.
\end{itemize}

\subsection{Subset Sum Resistance}
Subset sum analysis works on structured withdrawals that collectively match previous deposits. While it is probabilistic, it becomes more accurate when users follow predicatable withdrawal patterns or operate within narrow time windows.
\textbf{Recommended Countermeasure:}
\begin{itemize}
    \item \textbf{Withdrawal Amount Obfuscation:} Encourage users to withdraw in irregular amounts or add noise to avoid forming easily summable subsets.
    \item \textbf{Time-Based Delays:} Introduce randomized timing delays between deposits and corresponding withdrawals, reducing the effectiveness of temporal correlation in subset analyses.
    \item \textbf{Split and Merge Techniques:} Implement wallet level automation to split large deposits into several shielded notes and reassemble them internally before withdrawal, obscuring linkability at the transaction level.
\end{itemize}


\section{Conclusion}\label{sec:conclusion}
It is true that privacy preserving technologies such as Railgun represent a significant advancement in protecting user confidentiality on Ethereum, this work demonstrates that behavioral patterns can lead to deanonymization of users. Through a detailed analysis, we have shown that user practices, rather than cryptographic limitations often be the weakest link in the entire privacy system.
This analysis highlights the importance of building strong cryptographic protocols; however, ensuring their secure usage is equally as important. Our countermeasures offer some recommendations for developers and users to counter such analysis techniques and strengthen privacy guarantees.
In the end achieving anonymity on transparent blockchains requires approaches that combine cryptography, system design, and user behavior. As Zero knowledge based system continue to emerge, research is necessary to identify and address such threats, ensuring that privacy remains a reliable and important feature of decentralized ecosystems.
